Multi-modal Situated Reasoning in 3D Scenes

Situation awareness is essential for understanding and reasoning about 3D scenes in embodied AI agents. However, existing datasets and benchmarks for situated understanding are limited in data modality, diversity, scale, and task scope. To address these limitations, we propose Multi-modal Situated Question Answering (MSQA), a large-scale multi-modal situated reasoning dataset, scalably collected leveraging 3D scene graphs and vision-language models (VLMs) across a diverse range of real-world 3D scenes. MSQA includes 251K situated question-answering pairs across 9 distinct question categories, covering complex scenarios within 3D scenes. We introduce a novel interleaved multi-modal input setting in our benchmark to provide text, image, and point cloud for situation and question description, resolving ambiguity in previous single-modality convention (e.g., text). Additionally, we devise the Multi-modal Situated Next-step Navigation (MSNN) benchmark to evaluate models' situated reasoning for navigation. Comprehensive evaluations on MSQA and MSNN highlight the limitations of existing vision-language models and underscore the importance of handling multi-modal interleaved inputs and situation modeling. Experiments on data scaling and cross-domain transfer further demonstrate the efficacy of leveraging MSQA as a pre-training dataset for developing more powerful situated reasoning models.

==> Figure/figures/one_step_navigation_analysis.tex <==
% Table 3 on the left
\begin{table*}[ht]
\centering
\caption{SOTA on \shortnavi}
\setlength{\tabcolsep}{1mm}
\begin{tabular}{l|cccc|cc}
    \toprule
    Model & S & V & Settings &  PT data & Accuracy \\
    % & four - direction \\
    \midrule
    GPT-3.5 & T & OBJ & zero-shot & -- &  20.1 \\ %20.3 \\ % & 11.11 \\
    GPT-4o & T+I & OBJ & zero-shot & -- & 27.55 \\
    \midrule
    % \multirow{2}{*}{LEO} & T & PCD & from scratch & -- &  \\
    \multirow{2}{*}{LEO}  & T & PCD & FT &  LEO-align &  31.44 \\
      & T & PCD  & FT & \datasetname & 37.05\\
    \midrule
    \multirow{6}{*}{\modelname} & T+I & PCD & FT & -- & 45.46 \\
     & T & PCD & FT &  \datasetname & 45.61 \\
     % & T+I & PCD & FT + blind $\mathbf{P}$ &  \datasetname &    \\
     % & T+I & PCD & FT + blind $s^{txt,img}$ &  \datasetname &    \\
     & T+I & PCD & FT + test  &  \datasetname &  31.66 \\
      & T+I & PCD & FT & \datasetname &  \textbf{48.4} \\
    \bottomrule
\end{tabular}
\label{table:eval_one_step_nav}
\end{table*}

% Figure 7 and Table 4 stacked on the right
\begin{figure}[htbp]
    \centering
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/figures/scaling_effect_MSQA.png}
        \caption{Scaling effect on \datasetname}
        \label{fig:scaling_MSQA}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \captionof{table}{GPT-scores for cross domain transferring. The datasets on the left column denote the source domain, and the ones on the top row denote the target domain.}
        \vspace{1em} % Adjust space between caption and table
        \resizebox{\textwidth}{!}{
            \begin{tabular}{l|c|c|c}
            \toprule
                        & ScanNet & 3RScan & ARKit. \\
            \midrule
              ScanNet   & \textbf{55.40} & 43.33 & 52.16 \\
              3RScan    & 50.15 & \textbf{45.08} & 55.35 \\
              ARKit. & 40.08  & 40.07 & \textbf{63.34} \\
            \bottomrule
            \end{tabular}
        }
        \label{table:cross_domain_transfer}
    \end{minipage}
    \label{fig:scaling_effect}
\end{figure}

==> Figure/tex/QA_HOI_statistics.tex <==
% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.5\linewidth]{Figure/figures/QA_type_statistics.png}
%     \caption{Question type distribution.}
%     \label{fig:QA_type_statistics}
% \end{figure}

\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{0.29\textwidth}
        \includegraphics[width=1\textwidth]{Figure/figures/QA_distribution.pdf}
        \caption{Question types.}
        \label{fig:QA_type_distribution}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.25\textwidth}
        \includegraphics[width=\textwidth]{Figure/figures/HOI_distribution.pdf}
        \caption{HOI types.}
        \label{fig:HOI_type_distribution}
    \end{subfigure}
    \hfill
        \begin{subfigure}[b]{0.25\textwidth}
        \includegraphics[width=\textwidth]{Figure/figures/QA_dataset_distribution.pdf}
        \caption{Scene domains.}
        \label{fig:data_domain_distribution}
    \end{subfigure}
    \caption{MSQA statistics, including the distribution of question types, situation HOI types, and scene domains.}
    \label{fig:dataset_distribution}
\end{figure}

==> Figure/tex/scaling_and_one_step_navigation.tex <==
% Table 3 - State of the Art on one-step navigation
\begin{table}[htbp]
    \centering
    \caption{State of the Art on One-Step Navigation}
    \label{table:sota_one_step_nav}
    \begin{tabular}{l|cccc|c}
        \toprule
        Model & S & V & Settings & PT Data & Accuracy \\
        \midrule
        GPT-3.5 & T & OBJ & zero-shot & -- & 20.1 \\
        GPT-4+ & T+I & OBJ & zero-shot & -- & 27.55 \\
        \midrule
        LEO & T & PCD & FT & LEO-align & 31.44 \\
        & T & PCD & FT & MSQA & 37.05 \\
        \midrule
        MSR3D & T+I & PCD & FT & MSQA & 45.61 \\
        & T+I & PCD & FT + test & MSQA & 31.66 \\
        & T+I & PCD & FT & MSQA & \textbf{48.4} \\
        \bottomrule
    \end{tabular}
\end{table}

\vspace{2em} % Adjust the vertical space as needed

% Figure and Table for Scaling Effect and Cross-Domain Transfer
\begin{figure}[htbp]
    \centering
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/figures/scaling_effect_MSQA.png}
        \caption{Scaling effect on MSQA}
        \label{fig:scaling_MSQA}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \captionof{table}{GPT-scores for cross-domain transferring.}
        \label{table:cross_domain_transfer}
        \resizebox{\textwidth}{!}{
            \begin{tabular}{l|c|c|c}
                \toprule
                & ScanNet & 3RScan & ARKit. \\
                \midrule
                ScanNet & \textbf{55.40} & 43.33 & 52.16 \\
                3RScan & 50.15 & \textbf{45.08} & 55.35 \\
                ARKit. & 40.08 & 40.07 & \textbf{63.34} \\
                \bottomrule
            \end{tabular}
        }
    \end{minipage}
\end{figure}


==> Figure/tex/scaling_effect.tex <==
% \begin{figure}[htbp]
%     \centering
%     \begin{subfigure}[b]{0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figure/figures/scaling_effect_MSQA.png}
%         \caption{Scaling effect on \datasetname}
%         \label{fig:scaling_MSQA}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figure/figures/scaling_effect_One Step Navigation.png}
%         \caption{Scaling effect on one-step navigation}
%         \label{fig:scaling_one_step}
%     \end{subfigure}
%     \label{fig:scaling_effect}
% \end{figure}


\begin{figure}[htbp]
    \hfill
    \begin{minipage}[c]{0.48\textwidth}
        \centering
        \captionof{table}{GPT-scores for cross domain transferring. The datasets on the left column denote the source domain, and the ones on the top row denote the target domain.}
        \vspace{1em} % Adjust space between caption and table
        \resizebox{0.8\textwidth}{!}{
            \begin{tabular}{l|c|c|c}
            \toprule
                        & ScanNet & 3RScan & ARKit. \\
            \midrule
              ScanNet   & \textbf{55.40} & 43.33 & 52.16 \\
              3RScan    & 50.15 & \textbf{45.08} & 55.35 \\
              ARKit. & 40.08  & 40.07 & \textbf{63.34} \\
            \bottomrule
            \end{tabular}
        }
        \label{table:cross_domain_transfer}
    \end{minipage}
    \label{fig:scaling_effect}
\end{figure}




==> Table/SOTA_embodied_navi.tex <==
\begin{table}[t!]
\caption{Habitat object navigation performances of LEO against baselines. $^\dagger$ indicates zero-shot evaluation.}
\begin{tabular}{lcccccc}
\toprule
 \multicolumn{2}{c}{\multirow{2}{*}{}} & \multicolumn{2}{c}{\small{MP3D-val}} & & \multicolumn{2}{c}{\small{HM3D-val}} \\ \cmidrule(lr){3-4}\cmidrule(lr){6-7}
\multicolumn{2}{l}{} &  \small{Success$(\uparrow)$} & \small{SPL$(\uparrow)$} & & \small{Success$(\uparrow)$} &  \small{SPL$(\uparrow)$}\\ \midrule
\multicolumn{2}{c}{Habitat-web (shortest)~\cite{ramakrishnan2021habitat}} & 4.4 & 2.2 & & - &  - \\
\multicolumn{2}{c}{Habitat-web (demo)~\cite{ramakrishnan2021habitat}} & \textbf{35.4} & 10.2 & & - & - \\
% \multicolumn{2}{c}{VC-1 (ViT-B, demo)} & - & - & & \textbf{57.1} & \textbf{31.4} \\
% \multicolumn{2}{c}{CoW (\citeyear{gadre2023cows})} & 11.1$^\dagger$ & 6.3$^\dagger$ & & - & - \\
\multicolumn{2}{c}{ZSON~\cite{majumdar2022zson}} & 15.3$^\dagger$ & 4.8$^\dagger$ & & 25.5 & 12.6 \\

% \multicolumn{2}{c}{\agent w/o 3D} & 8.6 & 6.8 & - & - \\
% \multicolumn{2}{c}{\agent w/o 2D} & 7.8 & 4.6 & - & -  \\
\multicolumn{2}{c}{LEO~\cite{huang2023embodied}} & 23.1 & 15.2 & & 23.1$^\dagger$ & 19.1$^\dagger$ \\
\midrule
  % \multicolumn{2}{c}{\proposed-scratch} & fail & fail & & fail  & fail \\
\multicolumn{2}{c}{\modelname} & & & & & \\
\bottomrule
\end{tabular}
\end{table}

==> Table/SOTA_sqa.tex <==
\begin{table*}[t]
\centering
\caption{Comparison between \modelname and the SOTA methods on SQA3D dataset. Top-1 exact match accuracy is used as the metric for evaluation.}
\begin{tabular}{lcccccccccc}
    \toprule
      & \multicolumn{6}{c}{Question Type} & \multirow{2}{*}{Avg.}\\
     \cmidrule(lr){2-7}
     & What & Is & How & Can & Which & Others\\
    \midrule
    Scan2Cap(GPT-3)~\cite{chen2021scan2cap} & 39.7 & 46.0 & 40.5 & 45.6 & 36.1 & 38.4 & 41.0 \\
    ClipBERT~\cite{lei2021less} & 30.2 & 60.1 & 38.7 & 63.3 & 42.5 & 42.7 & 43.3 \\
    SQA3D~\cite{ma2023sqa3d} & 33.5 & \textbf{66.1} & 42.4 & 69.5 & 43.0 & 46.4 & 47.2 \\
    3D-VisTA~\cite{zhu20233d} & 34.8 & 63.3 & 45.4 & \textbf{69.8} & 47.2 & 48.1 & 48.5  \\
    3D-LLM~\cite{hong20233d} & 37.05 & 65.18 & 45.81 & 67.46 & 51.00 & 49.82 & 49.79 \\
    LEO~\cite{huang2023embodied} & - & - & - & - & - & - & 50.0 \\
    \midrule
    % \proposed-text & 38.19 & 66.41 & 46.67 & 68.64 & 49.00 & 50.58 & \textbf{50.58} \\
    % \proposed & 36.53 & 65.64 & \textbf{48.39} & 67.75 & \textbf{48.15} & \textbf{49.47} & \textbf{49.73} \\
    \modelname-scratch &  &  &  &  &  &  &  49.62  \\
    \modelname &  &  &  &  &  &  & 49.87  \\
    \modelname-text &  &  &  &  &  &  &  49.93  \\
    \modelname-scannet &  &  &  &  &  &  &      \\
    \bottomrule
\end{tabular}
\label{table:sqa_sota}
\end{table*}

==> Table/cross_domain_transfer.tex <==
\begin{table*}[t!]
% \small
\centering
\caption{GPT-scores for cross domain transferring. The datasets on the left column denote the source domain, and the ones on the top row denote the target domain.}
\small
% \setlength{\tabcolsep}{1mm}
\resizebox{0.6\linewidth}{!}{
    \begin{tabular}{l|c|c|c}
    \toprule
                & ScanNet & 3RScan & ARKit. \\
    \midrule
      ScanNet   & \textbf{55.40} & 43.33 & 52.16 \\
      3RScan    & 50.15 & \textbf{45.08} & 55.35 \\
      ARKit. & 40.08  & 40.07 & \textbf{63.34} \\
    \bottomrule
    \end{tabular}
}
\label{table:cross_domain_transfer}
\end{table*}


==> Table/data_quality_control_distribution_with_sqa.tex <==
\begin{table*}[ht]
\centering
\caption{Data scaling res on MSQA (maybe several figures) (GPT score as metrics)}
\setlength{\tabcolsep}{1mm}
\begin{tabular}{l|c|c|c|c}
    \toprule
     & average & 0-1 & scene \\
     \midrule
    1/8 &  \\
    1/4 &  \\
    1/2 &  \\
    full set &  \\
    \bottomrule
\end{tabular}

\label{table:data_quality_control_with_sqa}
\end{table*}

==> Table/data_scaling_msqa.tex <==
\begin{table*}[t!]
\centering
\caption{Data scaling res on MSQA (maybe several figures) (GPT score as metrics)}
\setlength{\tabcolsep}{1mm}
\begin{tabular}{l|c|c|c}
    \toprule
     & sitution & qa & scene \\
     \midrule
    1/8 & 51.31  & 50.64 & 51.72 \\
    1/4 & 52.90 & 52.04  & 52.86 \\
    1/2 & 53.59 & 53.59 & 53.62 \\
    full set & \textbf{54.13} & \textbf{54.13} & \textbf{54.13} \\
    \bottomrule
\end{tabular}

\label{table:data_scaling_msqa}
\end{table*}

==> Table/data_scaling_one_step.tex <==
\begin{table*}[t!]
\centering
\caption{Data scaling res on One step navigation (maybe several figures) (accuracy)}
\setlength{\tabcolsep}{1mm}
\begin{tabular}{l|cccccc}
    \toprule
    & \multicolumn{3}{c}{four direction} \\ % & \multicolumn{3}{c}{eight direction} \\
    & sitution & qa & scene \\ % & sitution & qa & scene \\
     \midrule
    from scratch  & \multicolumn{3}{c}{45.46} \\ % & \multicolumn{3}{c}{}\\
    1/8 & 46.15 & 45.12 & 46.29\\
    1/4 & 47.79 & 46.17 & 46.51\\
    1/2 &  & 46.36 & 48.21\\
    full set & \multicolumn{3}{c}{48.4} \\ % & \multicolumn{3}{c}{27.29} \\
    \bottomrule
\end{tabular}

\label{table:data_scaling_one_step_nav}
\end{table*}

==> Table/prompt_QA_generation.tex <==
\begin{figure*}[th!]\centering
\begin{minipage}{0.99\columnwidth}\vspace{0mm}    \centering
\begin{tcolorbox} 
\fontsize{9.0pt}{\baselineskip}\selectfont 
\blueprompt{object\_name} = \promptfromsample{object\_name} \\
\blueprompt{end\_situation} = \promptfromsample{end\_situation} \\
\blueprompt{examples} = "
    Given "Obejct description": { "relations": [ "to the left of table-35", "in front of shelf-56", "placed on floor-9" ], "attributes": { "color": "white", "3D shape": "rectangular prism", "material": "metal and plastic", "usage": "preserving food at low temperatures", "texture": "smooth", "structure": "upright, single-door", "state": "closed and functioning"}
    "object\_name": "refrigerator"}, 
    You can generate results like 
    "I want to open the white metal refrigerator.", 
    "I want to close the white refrigerator in front of the shelf."
    "I want to pick some food from the white refrigerator to the left of table." " \\
    \\
\blueprompt{prompt} = f""" \\
Please generate a sentence about doing something with the object \{\blueprompt{object\_name\}} based on the following information: 
Obejct attributes and spatial relationship descriptions are given in the following json: 
\{\blueprompt{end\_situation\}}, you can select part of the given information to generate the sentence. The generated sentence should be natural.
here is an example: \\
Object descriptions is \{\blueprompt{examples}\}
You can generate results like 
result: "I want to open the white metal refrigerator.", 
result: "I want to close the white refrigerator in front of the shelf."
result: "I want to pick some food from the white refrigerator to the left of table."
The generated results should be one sentence in the follow format like: result: ". \\
""" \\
\\
\textcolor{blue}{messages} = [\{"role": "user",  "content": [\{"type": "text", "text": \blueprompt{prompt}\}]
\end{tcolorbox}
\caption{Prompt messages to generate the goal action for \ac{mson}.}
\label{table::prompt_for_interaction}
\end{minipage}
\end{figure*}
